VALUE: Large Scale Voting-based Automatic Labelling for Urban Environments

This paper presents a simple and robust method for the automatic localisation of static 3D objects in large-scale urban environments. By exploiting the potential to merge a large volume of noisy but accurately localised 2D image data, we achieve superior performance in terms of both robustness and accuracy of the recovered 3D information. The method is based on a simple distributed voting schema which can be fully distributed and parallelised to scale to large-scale scenarios. To evaluate the method we collected city-scale data sets from New York City and San Francisco consisting of almost 400k images spanning the area of 40 km$^2$ and used it to accurately recover the 3D positions of traffic lights. We demonstrate a robust performance and also show that the solution improves in quality over time as the amount of data increases.

==> 6_discussion.tex <==
\section{Discussion}
\label{Discussion}

Table \ref{clusteringStats} presents the statistics of the computed clusters. Both maps have many views in each cluster, allowing for a better triangulation of contents. The average number of detections per view show that the detections are very noisy with many false positive which are filtered out by the system.

As shown in Table \ref{triangulationStatistics} we are able to detect at least 90\% of the traffic lights in both maps. The duplicates in both maps are not an issue given the merging step takes care of reducing them to one content. Wrong detections are mainly due to traffic light reflections on moving vehicles; these wrong detections can be filtered out by increasing the number of positive votes which are necessary to evaluate a content as positive, which has as disadvantage that more views of the same content might be necessary. The average reprojection error is low enough to have a good estimation of the traffic light position in space, given that we are aiming at detecting it's center. We computed all results using a reprojection factor of 1.0.

Figure \ref{fig:precision} shows the trade off between the number of triangulated contents and then reprojection error. Lowering the reprojection factor produces less contents with a higher accuracy. For example, a precision value of 0.1 produced 16 contents with a reprojection error of only 0.18 pixels while a precision value of 1.0 produced 172 content with a reprojeciton error of 2.94 as shown in table \ref{triangulationStatistics}.

==> UNUSED_evaluation.tex <==
\section{Experimental Results}
\label{Results}

The evaluation is performed following the organization of the work in detection and content matching as introduced in Section \ref{Method}. 

Three different aspects of the system have to be evaluated:
\begin{itemize}
 \item Detection: the accuracy of the traffic light detector has been assessed computing the intersection over union (IoU) on the training dataset as described in the work of Hoiem \emph{et Al.} \cite{hoiem2012diagnosing}. 
%  It has also been evaluated by comparing the detections in the evaluation maps with the detections produced by our system by re-projecting the output contents on the input images. 
\item Matching: evaluate the quality of the matching system which returns views of a given traffic light in all frames of the evaluation map. This had been done manually by checking all the matched views for each detected content. Each content has been evaluated as correct, incorrect or duplicate.
\item Triangulation: evaluate the quality of the triangulation system based on the quality of the matching system. Given that we don't have exact ground truth 3D positions for the traffic lights, we used the re-projection error and the \emph{root mean square} (RMS) to evaluate the system. We did this based on the quality of the matching system which is producing a large number of views for each traffic light as shown later in \ref{Results}.
% We also evaluated several multi view triangulation algorithms based on their reprojection error.
\end{itemize}

We evaluated the system on two different map, of which the second is larger than previously published results (1M images). 

\subsection{Data Sets}

The two evaluation maps, table \ref{table:datasets},  have been created using images captured from a moving car. Images were acquired using a mobile phone camera mounted on the windshield. The two evaluated maps are:
\begin{itemize}
\item A map of San Francisco around Union Square made of $\sim$25k frames. This map contains 183 traffic lights and covers an area of 3.2 square kilometers, with an elevation extent of 74m as shown in Figure \ref{fig:clusters}. Of all the traffic lights, we assume 167 as detectable, given that some traffic lights appear only in a few images or they are consistently occluded. 
\item A map of New York, mainly Manhattan, made of $\sim$1M frames of which 360628 were reconstructed in the map. This map contains 1906 traffic lights and covers an area of roughly 39.75 square kilometers with an extent of $13.19km \times 3.55km$ and elevation variation of 60m. There are 1732 detectable traffic lights in this map.
\end{itemize}

\begin{table}[ht]
\centering
\caption{Dataset statistics: standing frames are removed form the initial images. Images with detections are counted from the frames which were also reconstructed in the map.}
\label{table:datasets}
\begin{tabular}{|l|c|c|c|}
\hline
              & images & with detections & standing frames\\ \hline
San Francisco &      26825        &   7581     &  3562  \\ \hline
New York      &     1025928       &   103358   &  51411   \\ \hline
\end{tabular}
\end{table}

%\begin{figure}
%\includegraphics[width=\columnwidth]{images/map}
%\caption{First of the two maps used for the evaluation. This map is made of 25 thousand images.}
%\label{fig:map25k}
%\end{figure}

Both maps contain pedestrian traffic lights which were excluded from the analysis. In both maps the vehicle traveled the roads possibly multiple times and in both direction, at different times of the day and different weather conditions.

The standard deviation of the pose estimation of the above maps is $\sim$3cm based on undisclosed ground-truth verification.


